Strong-Separation Logic

Most automated verifiers for separation logic target the symbolic-heap fragment, disallowing both the magic-wand operator and the application of classical Boolean operators to spatial formulas. This is not surprising, as support for the magic wand quickly leads to undecidability, especially when combined with inductive predicates for reasoning about data structures. To circumvent these undecidability results, we propose to assign a more restrictive semantics to the separating conjunction. We argue that the resulting logic, strong-separation logic, can be used for compositional program verification and bi-abductive static analysis just like "standard" separation logic, while remaining decidable even in the presence of both the magic wand and the list-segment predicate -- a combination of features that leads to undecidability assuming the standard semantics.

==> images/ams-compose-example.tex <==
\newcommand{\RGone}{
      \begin{tikzpicture}
        \node[rgnode,label={}] (1) {$x$};
        \node[rgnode,below=7mm of 1,label={}] (2) {$y$};
        \node[rgnode,right=7mm of 1,label={}] (3) {$z,w$};
        \draw (1) edge[rgedge] node[above] {$\geqtwo$} (3);
        \draw (2) edge[rgedge] node[below,xshift=3mm,yshift=2mm] {$\eqone$} (3);
      \end{tikzpicture}
      }
    \newcommand{\RGtwo}{
        \begin{tikzpicture}
        \node[rgnode,label={}] (3) {$z,w$};
        \node[rgnode,below=7mm of 3,label={},xshift=3mm] (4) {$u$};
        \node[rgnode,right=7mm of 3,label={}] (5) {$v$};
        \draw (3) edge[rgedge] node[above] {$\eqone$} (5);
        \draw (4) edge[rgedge] node[below,xshift=3mm,yshift=2mm] {$\geqtwo$} (5);
      \end{tikzpicture}
      }
    \newcommand{\RGthree}{
      \begin{tikzpicture}
        \node[rgnode,label={}] (1) {$x$};
        \node[rgnode,below=7mm of 1,label={}] (2) {$y$};
        \node[rgnode,right=7mm of 1,label={}] (3) {$z,w$};
        \draw (1) edge[rgedge] node[above] {$\geqtwo$} (3);
        \draw (2) edge[rgedge] node[below,xshift=3mm,yshift=2mm] {$\eqone$} (3);
        %%
        %\node[rgnode,label={$z,w$}] (3) {3};
        \node[rgnode,below=7mm of 3,label={},xshift=3mm] (4) {$u$};
        \node[rgnode,right=7mm of 3,label={}] (5) {$v$};
        \draw (3) edge[rgedge] node[above] {$\eqone$} (5);
        \draw (4) edge[rgedge] node[below,xshift=3mm,yshift=2mm] {$\geqtwo$} (5);
      \end{tikzpicture}
    }
    \begin{tikzpicture}

      \node (ams1) {
      \tikzAMS{
        \RGone
      }{
        $\set{ \set{v} }$
      }{
        $1$
      }
    };

    \node[right=0mm of ams1] (compose) {\Huge$\Compose$};

    \node[right=0mm of compose] (ams2) {
      \tikzAMS{
        \RGtwo
      }{
        $\set{ \set{a,b} }$
      }{
        $3$
      }
    };

    \node[right=0mm of ams2] (eq) {\Huge$=$};

    \node[right=0mm of eq] (ams3) {
      \tikzAMS{
        \RGthree
      }{
        $\set{ \set{v}, \set{a,b}}$
      }{
        $4$
      }
      };
    \end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> proofs/algorithm-eq.tex <==
The truth of $x=y$ does not depend on the heap, so
      \[\set{\mabst\SH \mid \SH\ourmodels\phi}
        \cap \AMS_{\csize{\phi},\vec{x}} = \emptyset = \abst{\S}{x =
          y}\] if $\S(x)\neq\S(y)$ and
      \begin{align*}
        &\set{\mabst\SH \mid \H \in \HH \text{ and }\SH\ourmodels\phi}
        \cap \AMS_{\csize{\phi},\vec{x}}\\
        =& \set{\mabst\SH \mid \H \in \HH}
           \cap \AMS_{1,\vec{x}}\\
        =& \AMS_{1,\S} \\
        =& \abst{\S}{x=y}
      \end{align*}
      if $\S(x)=\S(y)$
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> proofs/algorithm-wedge.tex <==
\begin{description}
    \item[$\subseteq$]  Let $\A \in \abst{\S}{\phi_1\wedge\phi_2}$.
      %
      Let $\H$ be such that $\mabst\SH=\A$. (Such a heap must exist by
      Lemma~\ref{lem:ams:poly-models}.)
      %
      There then exist, by definition of
      $\boundcap{\csize{\phi_1}}{\csize{\phi_2}}$, for
      $1\leq i \leq 2$, AMS $\B_i$ such that
      $\B_i \in \abst{\S}{\phi_i}$ and
      $\A \in \lift{\csize{\phi_i}}{\csize{\phi_1 \wedge
          \phi_2}}{\B_i}$.
      %
      As $\A \kequivi{\csize{\phi_i}} \B_i$, it follows by
      Lemma~\ref{lem:mabstk:sound} that $\SH \ourmodels \phi_i$ iff
      there exists a heap $\H_i$ with $\SHi{i}\ourmodels\phi_i$ and
      $\mabst\SHi{i}=\B_i$. Such heaps do exist by the induction
      hypotheses.
      %
      Consequently, $\SH \ourmodels \phi_1$ and
      $\SH\ourmodels\phi_2$. By the semantics of $*$, this yields that
      $\SH \ourmodels \phi$.
    \item[$\supseteq$] Assume $\A \in \AMS_{\csize{\phi_1\wedge\phi_2},\vec{x}}$ and
    $\A=\mabst \SH$ for some $\SH$ with
    $\SH\ourmodels\phi_1\wedge\phi_2$. By the semantics of $*$,
    $\SH\ourmodels\phi_1$ and $\SH\ourmodels\phi_2$.
    %
    For $1\leq i \leq 2$, let $\B_i \in \AMS_{\csize{\phi_i},\vec{x}}$
    with $\B_i \kequivi{\csize{\phi_i} \A}$.
    %
    By the induction hypotheses $\B_i \in \abst{\S}{\phi_i}$.
    %
    Note that $\A \in \lift{\csize{\phi_i}}{\csize{\phi_1 \wedge
        \phi_2}}{\B_i}$.
    %
    Consequently, $\A \in \abst{\S}{\phi_1\wedge\phi_2}$.
  \end{description}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> proofs/ams-soundness-interesting-compact.tex <==
\paragraph*{Case $\phi_1*\phi_2$.}
    %
    \newcommand{\SHtwoprime}{\SHpair{\S}{\H_2'}}
    %
    By the semantics of $*$, there exist $\Hoo,\Hot$
    with $\H_1 = \Hoo \oursunion \Hot$,
    $\SHpair{\S}{\Hoo}\ourmodels \phi_1$, and
    $\SHpair{\S}{\Hot}\ourmodels \phi_2$.
    %
    Let $\A_1 := \mabst\SHpair{\S}{\Hoo}$ and
    $\A_2 := \mabst\SHpair{\S}{\Hot}$. By
    Lemma~\ref{lem:compose:correct},
    $\mabst\SHi{1} = \A_1 \Compose \A_2 = \mabst\SHi{2}$.
    %
    We apply Lemma~\ref{lem:decompose} to $\mabst\SHi{2}$,
    $\A_1$, and $\A_2$ to obtain heaps $\Hto,\Htt$ with
    $\H_2=\Hto\oursunion\Htt$, $\mabst\SHpair{\S}{\Hto}=\A_1$ and
    $\mabst\SHpair{\S}{\Hto}=\A_2$.

    For $1 \leq i \leq 2$, we apply the induction hypotheses for
    $\phi_i$, $\H_{1,i}$ and $\H_{2,i}$ to obtain that
    $\H_{2,i}\ourmodels\phi_i$.
    %
    By the semantics of $*$, we then have
    $\SHi{2}=\SHpair{\S}{\Hto \oursunion \Htt}\ourmodels
    \phi_1 * \phi_2$.
  %
  \paragraph*{Case $\phi_1 \sept \phi_2$.}
    %
    Since $\SHi{1}\ourmodels\phi_1\sept\phi_2$, there exists a heap
    $\H_0$ with $\SHpair{\S}{\H_0} \ourmodels \phi_1$ and
    $\SHpair{\S}{\H_1 \oursunion \H_0} \ourmodels \phi_2$.
    %
    We assume w.l.o.g.~that $\H_2\oursunion \H_0 \neq \bot$---if this
    is not the case, simply replace $\H_0$ with a heap $\H_0'$ with
    $\SHpair{\S}{\H_0}\Iso\SHpair{\S}{\H_0'}$ for which
    $\H_2\oursunion \H_0 \neq \bot$. By Lemma~\ref{lem:iso-same-sat},
    $\SHpair{\S}{\H_1 \oursunion \H_0'} \ourmodels \phi_2$.

    Note that $\mabst \SHpair{\S}{\H_1 \oursunion \H_0} =
    \mabst\SHi{1} \Compose \mabst\SHi{0} = \mabst\SHi{2} \Compose
    \mabst\SHi{0} = \mabst \SHpair{\S}{\H_2 \oursunion \H_0}$ (by
    assumption and Lemma~\ref{lem:compose:correct}).
    %
    It therefore follows from the induction hypothesis for $\phi_2$,
    $\SHpair{\S}{\H_1 \oursunion \H_0}$, and $\SHpair{\S}{\H_2
      \oursunion \H_0}$ that $\SHpair{\S}{\H_2 \oursunion
      \H_0}\ourmodels \phi_2$ and thus
    $\SHi{2}\ourmodels\phi_1\sept\phi_2$.
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> proofs/ams-soundness-interesting.tex <==
\item[Case $\phi_1*\phi_2$.]
    %
    \newcommand{\SHtwoprime}{\SHpair{\S}{\H_2'}}
    %
    By the semantics of $*$, there exist $\Hoo,\Hot$
    with $\H_1 = \Hoo \oursunion \Hot$,
    $\SHpair{\S}{\Hoo}\ourmodels \phi_1$, and
    $\SHpair{\S}{\Hot}\ourmodels \phi_2$.
    %
    Let $\A_1 := \mabst\SHpair{\S}{\Hoo}$ and
    $\A_2 := \mabst\SHpair{\S}{\Hot}$. By
    Lemma~\ref{lem:compose:correct},
    $\mabst\SHi{1} = \A_1 \Compose \A_2 = \mabst\SHi{2}$.
    %
    We can thus apply Lemma~\ref{lem:decompose} $\mabst\SHi{2}$,
    $\A_1$, and $\A_2$ to obtain heaps $\Hto,\Htt$ with
    $\H_2=\Hto\oursunion\Htt$, $\mabst\SHpair{\S}{\Hto}=\A_1$ and
    $\mabst\SHpair{\S}{\Hto}=\A_2$.

    For $1 \leq i \leq 2$, we apply the induction hypotheses for
    $\phi_i$, $\H_{1,i}$ and $\H_{2,i}$ to obtain that
    $\H_{2,i}\ourmodels\phi_i$.
    %
    By the semantics of $*$, we then have
    $\SHi{2}=\SHpair{\S}{\Hto \oursunion \Htt}\ourmodels
    \phi_1 * \phi_2$.
  %
  \item[Case $\phi_1 \sept \phi_2$.]
    %
    Since $\SHi{1}\ourmodels\phi_1\sept\phi_2$, there exists a heap
    $\H_0$ with $\SHpair{\S}{\H_0} \ourmodels \phi_1$ and
    $\SHpair{\S}{\H_1 \oursunion \H_0} \ourmodels \phi_2$.
    %
    We assume w.l.o.g.~that $\H_2\oursunion \H_0 \neq \bot$---if this
    is not the case, simply replace $\H_0$ with a heap $\H_0'$ with
    $\SHpair{\S}{\H_0}\Iso\SHpair{\S}{\H_0'}$ for which
    $\H_2\oursunion \H_0 \neq \bot$. By Lemma~\ref{lem:iso-same-sat},
    $\SHpair{\S}{\H_1 \oursunion \H_0'} \ourmodels \phi_2$.

    Note that $\mabst \SHpair{\S}{\H_1 \oursunion \H_0} =
    \mabst\SHi{1} \Compose \mabst\SHi{0} = \mabst\SHi{2} \Compose
    \mabst\SHi{0} = \mabst \SHpair{\S}{\H_2 \oursunion \H_0}$ (by
    assumption and Lemma~\ref{lem:compose:correct}).
    %
    It therefore follows from the induction hypothesis for $\phi_2$,
    $\SHpair{\S}{\H_1 \oursunion \H_0}$, and $\SHpair{\S}{\H_2
      \oursunion \H_0}$ that $\SHpair{\S}{\H_2 \oursunion
      \H_0}\ourmodels \phi_2$ and thus
    $\SHi{2}\ourmodels\phi_1\sept\phi_2$.
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> proofs/ams-soundness-proof.tex <==
Let
$\A := \AMquadruple$ be the AMS with
$\mabst\SHi{1} = \A = \mabst\SHi{2}$.
  %
  We proceed by induction on the structure of
  $\phi$.
  %
  We present only one direction of the proof, as the proof of the
  other direction is completely analogous. To this end, assume that
  the claim holds for all subformulas of $\phi$ and assume that
  $\SHi{1}\ourmodels \phi$.
  %
  In particular, this implies that $\A \in \phiabsts{\S}{\phi}$---a
  fact that we will use throughout this proof.
  %
  We need to show that $\SHi{2}\ourmodels \phi$.
  \begin{description}
  \item[Case $\emp$.]  By Lemma~\ref{lem:phiabst:emp}, $\E=\emptyset$,
    $\Rset=\emptyset$, and $\garb=0$.
    %
    Consequently, $\H_2$ consists of zero chunks, i.e.,
    $\H_2=\emptyset$ and $\SHi{2}\ourmodels\emp$.
    %
  \item[Case $x \pto y$.]  By Lemma~\ref{lem:phiabst:emp},
    $\E=\set{\eqclass{\S}{x} \mapsto (\eqclass{\S}{y}, \eqone)}$,
    $\Rset=\emptyset$, and $\garb=0$.
    %
    Consequently, $\H_2 = \set{\S(x)\mapsto\S(y)}$
    %
    By the semantics of points-to assertions, it follows that
    $\SHi{2}\ourmodels x \pto y$.
    %
  \item[Case $\ls(x,y)$.]  By Lemma~\ref{lem:phiabst:ls}, $\A$ is an
    abstract list segment.
    %
    Consequently, there exist $z_1,\ldots,z_n$ such that $x=z_1$,
    $y=z_n$, and $\H_2$ consists of $n-1$ path chunks
    $\H_{2,1},\ldots,\H_{2,n-1}$ with
    $z_i \in \rootvars{\S}{\H_{2,i}}$ and
    $z_{i+1} \in \sinkvars{\S}{\H_{2,i}}$.
    %
    There are two cases.
    \begin{enumerate}
    \item $n=1$. In this case $x=y$ and the heap consists of zero
      chunks, i.e., of an empty list. Thus,
      $\SHi{2}\ourmodels\ls(x,y)$
    \item $n>1$.  In this case, we observe that since all path chunks
      are connected (the root variables of chunk $i+1$ are the sink
      variables of chunk $i$), the $x \in \rootvars{\S}{\H_{2,1}}$,
      and $y \in \sinkvars{\S}{\H_{2,n-1}}$, it follows that
      $\SHi{2}\ourmodels\ls(x,y)$.
    \end{enumerate}
    %
  \item[Case $x=y$.]  It follows from Lemma~\ref{lem:phiabst:eq} that
    $\eqclass{\S}{x}=\eqclass{\S}{y}$ and thus
    $\SHi{2}\ourmodels x=y$.
    %
  \input{proofs/ams-soundness-interesting}
    %
  \item[Case $\phi_1 \wedge \phi_2$.]
    By the semantics of $\wedge$, we have $\SHi{1}\ourmodels \phi_1$
    and $\SHi{1}\ourmodels \phi_2$.
    %
    We apply the induction hypotheses for $\phi_1$ and
    $\phi_2$ to obtain $\SHi{2}\ourmodels \phi_1$ and
    $\SHi{2}\ourmodels \phi_2$.
    %
    By the semantics of $\wedge$, we then have
    $\SHi{2}\ourmodels\phi_1\wedge\phi_2$.
  \item[Case $\phi_1 \vee \phi_2$.] By the semantics of $\vee$, we
    have $\SHi{1}\ourmodels \phi_1$ or $\SHi{1}\ourmodels
    \phi_2$. Assume w.l.o.g.~that $\SHi{1}\ourmodels\phi_1$.  We apply
    the induction hypothesis for $\phi_1$ to obtain
    $\SHi{2}\ourmodels \phi_1$.
    %
    By the semantics of $\vee$, we then have
    $\SHi{2}\ourmodels\phi_1\vee\phi_2$.
  \item[Case $\neg \phi_1$.] By the semantics of $\neg$, we have
    $\SHi{1}\not\ourmodels \phi_1$.
    %
    By the induction hypothesis for
    $\phi_1$ we then obtain $\SHi{2}\not\ourmodels \phi_1$.
    %
    By the semantics of $\neg$, we have
    $\SHi{2}\ourmodels\neg\phi_1$.
    \qedhere
  \end{description}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tablesandfigures/syntax-positive.tex <==
\[
  \begin{array}{lll}
    \atomic & ::= & \emp \mid x \pto y \mid \ls(x,y) \mid x = y \\
    \phi & ::= & \atomic \mid \phi * \phi \mid \phi \sept \phi \mid \phi \wedge \phi \mid \phi \vee \phi
  \end{array}
\]

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

